Visualization of atomistic optical waves in crystals

The refractive index of a matter is foundational to quantify the light-matter interaction of the medium. However, the classical description of refractive index is based on macroscopic homogenization and is limited to describing the local optical response of materials. A complete quantum description of light-matter interaction should consider nonlocality and multiple-scattering of optical responses at the atomistic lattice level. Recently, the deep microscopic optical band structure was introduced as a quantum generalization of refractive index of a medium. This quantum description unveils multiple optical eigenmodes in crystalline solids and hidden microscopic optical waves at the lattice level. In this work, we unravel the microscopic optical waves in silicon carbide. We predict and visualize hidden microscopic optical eigenwaves, which can be nonplanar and inhomogeneous even near the optical limit. Also, the nonlocal macroscopic dielectric constant of the crystal is analyzed using the microscopic optical waves as the basis. Our work establishes a general framework for picoscale electrodynamics applicable to other materials including two-dimensional materials.

==> old/__recycle_bin.tex <==


 % polarization and refractive index
    In classical electrodynamics, the concept of refractive index has explained how light interacts with and behaves inside a macroscopic homogeneous material \cite{jackson1999}. This concept has successfully represented the optical properties of materials, enabling the demonstration of various optical devices in imaging, optical sensors, and nano-optics. Such homogenization scheme has been extended beyond atomic scale to subwavelength scale, and metamaterials have been actively researched for exotic and unnatural optical properties including negative refractive index, optical magnetism, and artificial chirality.
%
However, recent advances on photonic crystals and resonant meta-optics  have reached the regimes with strong spatial nonlocality where the classical homogenization fails \cite{tsukerman2017}. It is now clear that the concept of refractive index needs to be more generalized 

what about natural (atomic) materials?
% \cite{kim2016,kim2017}
% \cite{shim2021,andreoli2021}
% \cite{mao2021,jung2022}


nonlocality has often been neglected

recent investigations ++
strong nonlocality
nonlocal hydrodynamic 


intrinsic (hidden) waves exist in a crystal



    
    The question is: how light propagates inside a material? - or how material responses to light?

spatial nonlocality

    refractive index is introduced to ++ light propagation in a dielectric material
refractive index ++ the ratio of the speed of light in the vacuum to the effective speed in the material

    $n(\omega) = \sqrt{\varepsilon(\omega)} = \sqrt{1+\chi(\omega)}$, where $\varepsilon$ and $\chi$ are the relative permittivity and the electric susceptibility of the material, respectively, and the magnetic response is ignored with ($\mu = 1$).

    the electric susceptibility is the measure of how material responses (polarizes) to the incoming electromagnetic fields,
    % quantify the light-matter interaction of the material?
    how light propagates inside the material is intimately related to this response (as refractive index)

    However, this description has been limited to classical macroscopic, uniform fields. 
    % why microscopic description is required?
    Because electromagnetic fields inside a crystalline solid experience atomic lattices as the inhomogeneities in the sub-nanometer scale, the microscopic fields are rapidly-varying at the atomic scale. 
        
    local-field effects
    nonlocality
    ++momentum exchange
    
    
    %modern theory of polarization
    the state-of-the-art understanding on polarization
    Berry-Vanderbilt-Resta theory of polarization\cite{king1993,resta1993}
    but limited to macroscopic, static 
    incapable of treating the dynamic optical responses of crystalline solids  

  %Claussius-Mossotti
    Claussius-Mossotti(-Lorentz-Lorentz) description related microscopic polarizability to macroscopic dielectric constant, 
    but limited to classical, ++ local
    

    nonlocal hydrodynamic

    metamaterials


    
    % novelty of this work?
   Therefore, we aim to investigate the dynamic optical polarization at the atomistic lattice level as general physical quantity representing optical characteristics of the material, analogous to electronic wavefunctions representing electronic characteristics. Specifically, we investigate this so-called optical pico-polarization in a realistic semiconductor material of silicon carbide (SiC) for its technological importance [+REF]. 

    We also examine the transverse optical responses, which have often been ignored in the literature, despite the transversality of light in the free space. 
    % purpose of this article?
    We hope this article will 



    
    \subsection{Atomistic polarization waves in a crystalline solid and their associated optical-indices}
    In this section, we investigate the optical responses of a crystalline solid at the atomistic level, and discuss the optical waves associated with the lattice. Analogous to the classical macroscopic polarization $4\pi\mathbf{P}(\omega)=\chi(\omega)\mathbf{E}(\omega)$, where $\chi$ is susceptibility, the microscopic polarization could be expressed as $4\pi\mathbf{p}_{\mathbf{g}}(\mathbf{q},\omega)=\sum_{\mathbf{g'}}\chi_{\mathbf{gg'}}(\mathbf{q},\omega)\mathbf{E}_\mathbf{g'}(\mathbf{q},\omega)$, where $\chi_{\mathbf{gg'}}(\mathbf{q},\omega)$ is the atomistic lattice susceptibility matrix and $\mathbf{g}$ is the reciprocal lattice vector of the crystalline solid.  However, this expression of polarization involves a predefined electric field and thus cannot fully represent the intrinsic optical properties of the material. In fact,  the susceptibility matrix contains all optical responses of the material including its symmetry, but the information is hidden behind its complexity. 
    
    One way to probe this hidden material information is the eigen-decomposition of the susceptibility matrix, and we express the polarization waves as
    \begin{equation}
        4\pi\mathbf{p}_{\lambda}^{L}(\mathbf{r},\mathbf{q},\omega) = \alpha_{\lambda}^{L}(\mathbf{q},\omega) \sum_{\mathbf{g}} e^{i(\mathbf{g+q})\cdot\mathbf{r}} \mathbf{n}_{\mathbf{g+q}}\tilde{p}_{\lambda}^{L}(\mathbf{g+q},\omega),
    \end{equation}
    where $\alpha_{\lambda}^{L}$ and $\tilde{p}_{\lambda}^{L}$ are the eigenvalues and eigenvectors of the susceptibility matrix $\chi_{\mathbf{gg'}}^{L}$. The superscript $L$ indicates the longitudinal fields with the normal unit vector $\mathbf{n}_{\mathbf{g+q}} = \frac{\mathbf{g+q}}{|\mathbf{g+q}|}$, such that $\nabla\times\mathbf{p}_{\lambda}^{L}=0$.  For cubic materials including zinc-blende crystals, the longitudinal and transverse responses can be decoupled and considered separately. The transverse fields can be similarly considered with the tangential unit vector $\mathbf{t}_{\mathbf{g+q}}$, such that $\mathbf{n}_{\mathbf{g+q}}\cdot\mathbf{t}_{\mathbf{g+q}}$ and $\nabla\cdot\mathbf{p}_{\lambda}^{T}=0$. The longitudinal and transverse lattice susceptibility matrices can be obtained under the random-phase approximation and perturbation theory\cite{adler1962,wiser1963,bharadwaj2022}.

    
    -----
    
    % analogy to the refractive index?
     The physical meaning of the optical-index is the strength of light-matter interaction in a material analogous to the susceptibility $\chi$. 
In the classical optics limit with small momentum $|\mathbf{q}|$ indicated by the shaded regions in Fig.~\ref{fig:2}d and \ref{fig:2}e, the optical-index can be related to the refractive index as $n(\omega)=\sqrt{1+\alpha_{\lambda=0}(|\mathbf{q}|\rightarrow0,\omega)}$. 
    
    In the classical macroscopic limit, the refractive index is obtained as $n = \sqrt{1+\chi}$

    refractive index increases as the material is more strongly polarized


    similarly, the physical meaning of the pico-index is how strong the material responses to the light


the pico-polarization waves $\mathbf{p}_{\lambda}$ represent the ++ associated with the optical-index $\alpha_{\lambda}$

The number of the pico-polarization bands is infinite, but the susceptibility matrix is truncated to a ++


the form of susceptibility matrix with different symmetry groups (in SI)




    % whay is the physical meaning of refractive index?
    Classical macroscopic limit-> 
    refractive index is related to the wavelength of light inside the material $\lambda = \lambda_0/n$
    
    % symmetry, degeneracy
    The lattice susceptibility 
    
    Two degeneracy at $L$-point

    Three degeneracy at $\Gamma$-point

    Two degeneracy at $X$-point

    The same number of degeneracy are observed for the valence bands of the electronic waves (the four lower energy bands in Fig.~\ref{fig:2}a).
    % ref Supporting figures for the degeneracy appearing in distribution


    \subsection{Longitudinal and transverse optical pico-polarization waves}
    
    -- Figure X


    In this section, we examine the 

    The dominant band ($\lambda=0$) near the $\Gamma$-point represents the classical optical limit, and the polarization density distribution looks like a simple planewave (Fig.~\ref{fig:p_L_dist}a). 
    Away from the $\Gamma$-point, the optical pico-polarization waves can be strongly distorted. This is shown with the optical polarization density distribution at K-point (Fig.~\ref{fig:p_L_dist}b). Such rapidly-varying polarization density distribution at the subwavelength level comes from the optical responses at the lattice level associated with the local-field effect, or the momentum exchange processes involving hte atomic lattice diffractions. 

The optical pico-polarization wave density distributions and their vector plots are given in the Supporting Materials. 

    %-- Figure X
    % transverse~~






    % towards experimental measurements? can we get something new (not just mere interpretation) observation based on this description?

    \clearpage
    \section{\label{sec:3}Discussion and Conclusion}
    
    Main text:
    - brief mention of picomax
    - symmetry?
    - brief mention of phonon?
    - brief mention of optical dispersion, plasmon dispersion, ...
    
    discuss how to access those ++
    {it is important that this new theory has to provide some unknown or new information that the previous theories could not provide. Also, how to experimentally access those info. }
    
    
    Appendix:
    - dielectric matrix eq. + results
    - local-field directions
    - polarization distribution at all symmetry points
    -+ lattice nonlocal Ohm's law
    
    Relevant groups? theoreticalspectroscopy group, 







% \begin{figure}
%     \centering
%     \includegraphics[scale=0.5]{fig4.pdf}
%     \caption{The distributions of the dominant ($\lambda=0$) dielectric eigenwaves of a crystalline solid at different high-symmetry points. (a) $\Gamma$-point, (b) X-point, (c) L-point; (i) The density of the eigenwaves (top row) and (ii) the contour plot of the real part of the induced charge density distributions (bottom row). The surface color of the induced charge density indicates its sign; red: positive, blue: negative. The induced charge density oscillates in time, and the plotted real part is a snapshot in an arbitrary time. The red arrow indicates the direction of the crystal momentum \textbf{q}. The crystal momentum at the $\Gamma$-point is $\mathbf{q}=\frac{2\pi}{a}(10^{-6},0,0)$. Frequency is at $\omega$ = 10~THz.}
%     \label{fig:4}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[scale=0.5]{fig5.pdf}
%     \caption{The distributions of the higher-order eigenwaves ($\lambda>0$) at the $\Gamma$-point. (a-f) The contour plots of the real part of the induced charge density distributions of higher-order eigenwaves with $\lambda=1$ to 6. The eigenwaves with $\lambda=1$  and 2 have degenerate screening strengths, so their distributions are similar. The green solid arrow in $\lambda=4$ indicates the polarization direction parallel to the crystal momentum, allowing this eigenwave to have strong coupling with a macroscopic planewave. The crystal momentum at the $\Gamma$-point is . Frequency is at $\omega$ = 10~THz. }
%     \label{fig:5}
% \end{figure}
